HATS-50b through HATS-53b: four transiting hot Jupiters orbiting G-type stars discovered by the HATSouth survey

We report the discovery of four close-in transiting exoplanets, HATS-50 through HATS-53, discovered using the HATSouth three-continent network of homogeneous and automated telescopes. These new exoplanets belong to the class of hot Jupiters and orbit G-type dwarf stars, with brightness in the range V=12.5-14.0 mag. While HATS-53 has many physical characteristics similar to the Sun, the other three stars appear to be metal rich, larger and more massive. Three of the new exoplanets, namely HATS-50, HATS-51 and HATS-53, have low density and similar orbital period. Instead, HATS-52 is more dense and has a shorter orbital period. It also receives an intensive radiation from its parent star and, consequently, presents a high equilibrium temperature. HATS-50 shows a marginal additional transit feature consistent with an ultra-short period hot super Neptune, which will be able to be confirmed with TESS photometry.

==> HATS580-019_rvtable.tex <==
$ 6828.86592 $ & $   -17.38 $ & $    24.00 $ & $   75.0 $ & $   37.0 $ & $   0.168 $ & Coralie \\
$ 6829.74512 $ & $    24.62 $ & $    26.00 $ & $  118.0 $ & $   43.0 $ & $   0.398 $ & Coralie \\
$ 6857.78434 $ & $    68.26 $ & $    12.00 $ & $    9.0 $ & $   15.0 $ & $   0.719 $ & FEROS \\
$ 6858.73766 $ & $    14.26 $ & $    11.00 $ & $   11.0 $ & $   14.0 $ & $   0.968 $ & FEROS \\
$ 6859.76731 $ & $   -56.74 $ & $    12.00 $ & $    4.0 $ & $   16.0 $ & $   0.237 $ & FEROS \\
$ 6862.68928 $\tablenotemark{d} & $   144.26 $ & $    33.00 $ & $   50.0 $ & $   41.0 $ & $   0.000 $ & FEROS \\
$ 6907.82693 $ & $    58.01 $ & $     4.95 $ & \nodata      & \nodata      & $   0.786 $ & HIRES \\
$ 6908.75386 $ & $    31.96 $ & $     5.67 $ & \nodata      & \nodata      & $   0.028 $ & HIRES \\
$ 6909.74379 $ & $    -4.97 $ & $    11.27 $ & \nodata      & \nodata      & $   0.287 $ & HIRES \\
$ 6911.50060 $ & $   -62.38 $ & $    41.00 $ & $ -301.0 $ & $   63.0 $ & $   0.746 $ & Coralie \\
$ 6911.76564 $ & $    49.40 $ & $     4.49 $ & \nodata      & \nodata      & $   0.815 $ & HIRES \\
$ 6912.49456 $\tablenotemark{d} & $   -62.38 $ & $    30.00 $ & $ -178.0 $ & $   51.0 $ & $   0.005 $ & Coralie \\
$ 6912.79856 $ & $   -36.69 $ & $     4.79 $ & \nodata      & \nodata      & $   0.084 $ & HIRES \\
$ 6913.78648 $ & $   -68.78 $ & $     5.12 $ & \nodata      & \nodata      & $   0.342 $ & HIRES \\
$ 6932.53890 $ & $  -176.74 $ & $    13.00 $ & $  -75.0 $ & $   17.0 $ & $   0.239 $ & FEROS \\
$ 6942.60598 $ & $     0.26 $ & $    13.00 $ & $  -29.0 $ & $   16.0 $ & $   0.868 $ & FEROS \\
$ 6983.54362 $ & $    67.26 $ & $    11.00 $ & $   23.0 $ & $   15.0 $ & $   0.557 $ & FEROS \\
$ 7166.81632 $ & $   -64.74 $ & $    15.00 $ & $  -30.0 $ & $   19.0 $ & $   0.413 $ & FEROS \\
$ 7181.70212 $ & $    -3.74 $ & $    14.00 $ & $    8.0 $ & $   18.0 $ & $   0.300 $ & FEROS \\
$ 7186.89313 $ & $   112.26 $ & $    18.00 $ & $   75.0 $ & $   24.0 $ & $   0.655 $ & FEROS \\
$ 7188.70636 $ & $   -22.74 $ & $    13.00 $ & $   15.0 $ & $   18.0 $ & $   0.129 $ & FEROS \\
$ 7209.04868 $ & $     1.46 $ & $     6.60 $ & \nodata      & \nodata      & $   0.440 $ & HIRES \\
$ 7211.80755 $ & $   -45.74 $ & $    12.00 $ & $   21.0 $ & $   16.0 $ & $   0.161 $ & FEROS \\
$ 7219.64476 $ & $   -47.74 $ & $    12.00 $ & $  -19.0 $ & $   17.0 $ & $   0.207 $ & FEROS \\
$ 7223.64984 $ & $     6.26 $ & $    15.00 $ & $   36.0 $ & $   20.0 $ & $   0.253 $ & FEROS \\
$ 7225.55693 $ & $    62.26 $ & $    11.00 $ & $  -11.0 $ & $   15.0 $ & $   0.751 $ & FEROS \\
$ 7227.54760 $ & $   -73.74 $ & $    13.00 $ & $  -41.0 $ & $   17.0 $ & $   0.271 $ & FEROS \\
$ 7235.52005 $ & $  -191.74 $ & $    34.00 $ & $   99.0 $ & $   20.0 $ & $   0.352 $ & FEROS \\
$ 7236.84001 $ & $  -114.74 $ & $    17.00 $ & $  129.0 $ & $   19.0 $ & $   0.697 $ & FEROS \\
$ 7297.66592 $ & $   -52.74 $ & $    18.00 $ & $ -177.0 $ & $   24.0 $ & $   0.580 $ & FEROS \\
$ 7299.64213 $ & $   -83.74 $ & $    16.00 $ & $  -16.0 $ & $   22.0 $ & $   0.096 $ & FEROS \\
$ 7557.80118 $ & $    62.26 $ & $    12.00 $ & $  -28.0 $ & $   17.0 $ & $   0.505 $ & FEROS \\
$ 7558.81095 $ & $    80.26 $ & $    12.00 $ & $   33.0 $ & $   17.0 $ & $   0.769 $ & FEROS \\
$ 7569.65730 $ & $   106.26 $ & $    15.00 $ & $   93.0 $ & $   22.0 $ & $   0.601 $ & FEROS \\
$ 7576.64710 $ & $    41.26 $ & $    16.00 $ & $   39.0 $ & $   21.0 $ & $   0.426 $ & FEROS \\
$ 7590.72922 $ & $   -25.94 $ & $    10.50 $ & $   22.0 $ & $   14.0 $ & $   0.103 $ & FEROS \\
$ 7593.67838 $ & $     4.86 $ & $    12.90 $ & $   54.0 $ & $   17.0 $ & $   0.874 $ & FEROS \\
$ 7612.71943 $ & $   113.86 $ & $    12.30 $ & $    6.0 $ & $   17.0 $ & $   0.845 $ & FEROS \\
$ 7614.57198 $ & $    79.66 $ & $    12.60 $ & $  127.0 $ & $   16.0 $ & $   0.329 $ & FEROS \\


==> HATS601-050_rvtable.tex <==
$ 6939.83172 $ & $   -15.58 $ & $    17.00 $ & $  -11.0 $ & $   27.0 $ & $   0.491 $ & Coralie \\
$ 6940.81069 $ & $   104.42 $ & $    63.00 $ & $    5.0 $ & $   68.0 $ & $   0.783 $ & Coralie \\
$ 6941.86563 $ & $   -73.58 $ & $    19.00 $ & $  -60.0 $ & $   29.0 $ & $   0.098 $ & Coralie \\
$ 6967.78670 $ & $   132.42 $ & $    19.00 $ & $  116.0 $ & $   29.0 $ & $   0.838 $ & Coralie \\
$ 6969.79828 $ & $    30.42 $ & $    18.00 $ & $   23.0 $ & $   27.0 $ & $   0.439 $ & Coralie \\
$ 6972.69347 $ & $   -50.58 $ & $    16.00 $ & $   65.0 $ & $   25.0 $ & $   0.303 $ & Coralie \\
$ 6997.69160 $ & $   178.26 $ & $    10.00 $ & $   87.0 $ & $   12.0 $ & $   0.768 $ & FEROS \\
$ 6997.73191 $ & $   201.26 $ & $    10.00 $ & $   74.0 $ & $   13.0 $ & $   0.780 $ & FEROS \\
$ 6999.63851 $ & $    -9.74 $ & $    10.00 $ & $   38.0 $ & $   11.0 $ & $   0.349 $ & FEROS \\
$ 7030.81040 $ & $    36.26 $ & $    10.00 $ & $    2.0 $ & $   10.0 $ & $   0.657 $ & FEROS \\
$ 7033.73624 $ & $     3.26 $ & $    10.00 $ & $    9.0 $ & $   10.0 $ & $   0.531 $ & FEROS \\
$ 7035.75138 $ & $   -68.74 $ & $    10.00 $ & $   -4.0 $ & $   11.0 $ & $   0.133 $ & FEROS \\
$ 7036.67747 $ & $   -49.74 $ & $    10.00 $ & $    6.0 $ & $   10.0 $ & $   0.409 $ & FEROS \\
$ 7037.79634 $ & $    59.26 $ & $    10.00 $ & $   12.0 $ & $   10.0 $ & $   0.744 $ & FEROS \\
$ 7049.60146 $ & $   -96.74 $ & $    10.00 $ & $  -22.0 $ & $   10.0 $ & $   0.269 $ & FEROS \\
$ 7050.67770 $ & $    34.26 $ & $    10.00 $ & $   12.0 $ & $   10.0 $ & $   0.590 $ & FEROS \\
$ 7053.74327 $ & $   -17.74 $ & $    10.00 $ & $  -18.0 $ & $   10.0 $ & $   0.505 $ & FEROS \\
$ 7054.60465 $ & $    61.26 $ & $    10.00 $ & $   -5.0 $ & $   10.0 $ & $   0.763 $ & FEROS \\
$ 7055.64520 $ & $   -94.74 $ & $    10.00 $ & $  -65.0 $ & $   10.0 $ & $   0.073 $ & FEROS \\
$ 7057.74745 $ & $     8.26 $ & $    10.00 $ & $  -85.0 $ & $   11.0 $ & $   0.701 $ & FEROS \\
$ 7075.63657 $ & $   -61.58 $ & $    18.00 $ & $    6.0 $ & $   29.0 $ & $   0.043 $ & Coralie \\
$ 7076.65198 $ & $   -86.58 $ & $    18.00 $ & $   -2.0 $ & $   29.0 $ & $   0.346 $ & Coralie \\
$ 7078.63334 $ & $    -0.58 $ & $    18.00 $ & $  -46.0 $ & $   29.0 $ & $   0.938 $ & Coralie \\
$ 7080.99763 $ & $    18.92 $ & $     9.40 $ & \nodata      & \nodata      & $   0.644 $ & CYCLOPS \\
$ 7081.01370 $ & $    42.82 $ & $     6.40 $ & \nodata      & \nodata      & $   0.649 $ & CYCLOPS \\
$ 7081.07820 $ & $    59.12 $ & $     8.60 $ & \nodata      & \nodata      & $   0.668 $ & CYCLOPS \\
$ 7082.97896 $ & $   -58.38 $ & $     9.00 $ & \nodata      & \nodata      & $   0.235 $ & CYCLOPS \\
$ 7082.99492 $ & $   -49.68 $ & $     7.60 $ & \nodata      & \nodata      & $   0.240 $ & CYCLOPS \\
$ 7083.01087 $ & $   -34.78 $ & $    11.70 $ & \nodata      & \nodata      & $   0.245 $ & CYCLOPS \\
$ 7149.86599 $ & $  -104.58 $ & $    13.50 $ & \nodata      & \nodata      & $   0.208 $ & CYCLOPS \\
$ 7149.89323 $ & $  -100.98 $ & $    13.00 $ & \nodata      & \nodata      & $   0.217 $ & CYCLOPS \\
$ 7149.90918 $ & $  -123.48 $ & $    20.90 $ & \nodata      & \nodata      & $   0.221 $ & CYCLOPS \\
$ 7152.85935 $ & $   -57.48 $ & $    12.10 $ & \nodata      & \nodata      & $   0.102 $ & CYCLOPS \\
$ 7152.86772 $ & $   -72.48 $ & $    20.40 $ & \nodata      & \nodata      & $   0.105 $ & CYCLOPS \\
$ 7154.86321 $ & $    77.12 $ & $     5.30 $ & \nodata      & \nodata      & $   0.701 $ & CYCLOPS \\
$ 7154.87917 $ & $   113.72 $ & $     6.70 $ & \nodata      & \nodata      & $   0.705 $ & CYCLOPS \\
$ 7313.71457 $ & $    -4.58 $ & $    18.00 $ & $  147.0 $ & $   49.0 $ & $   0.135 $ & Coralie \\
$ 7317.75708 $ & $  -228.58 $ & $    19.00 $ & $  -74.0 $ & $   38.0 $ & $   0.342 $ & Coralie \\
$ 7318.73072 $ & $    53.42 $ & $    18.00 $ & $  -27.0 $ & $   38.0 $ & $   0.633 $ & Coralie \\
$ 7408.69120 $ & $   -28.58 $ & $    12.00 $ & $   16.0 $ & $   20.0 $ & $   0.496 $ & Coralie \\
$ 7409.69015 $ & $    14.42 $ & $    12.00 $ & $   10.0 $ & $   20.0 $ & $   0.794 $ & Coralie \\
$ 7410.58904 $ & $    82.42 $ & $    14.00 $ & $  -92.0 $ & $   23.0 $ & $   0.063 $ & Coralie \\
$ 7411.54533 $ & $   -88.58 $ & $    19.00 $ & $ -141.0 $ & $   32.0 $ & $   0.348 $ & Coralie \\
$ 7464.64412 $ & $   -70.58 $ & $    17.00 $ & $  -54.0 $ & $   32.0 $ & $   0.204 $ & Coralie \\
$ 7466.52399 $ & $    82.42 $ & $    17.00 $ & $   25.0 $ & $   29.0 $ & $   0.765 $ & Coralie \\
$ 7640.86434 $ & $    63.42 $ & $    16.00 $ & $   23.0 $ & $   29.0 $ & $   0.825 $ & Coralie \\
$ 7643.82622 $ & $    61.42 $ & $    13.00 $ & $  -23.0 $ & $   26.0 $ & $   0.709 $ & Coralie \\
$ 7645.89470 $ & $   -50.58 $ & $    12.00 $ & $    4.0 $ & $   22.0 $ & $   0.327 $ & Coralie \\


==> HATS606-028_rvtable.tex <==
$ 7109.65449 $ & $  -323.80 $ & $    34.00 $ & $\cdots$ & $\cdots$ & $   0.165 $ & Coralie \\
$ 7118.61984 $ & $   378.20 $ & $    24.00 $ & $  -15.0 $ & $   31.0 $ & $   0.725 $ & HARPS \\
$ 7119.61676 $ & $   -82.80 $ & $    31.00 $ & $   95.0 $ & $   37.0 $ & $   0.455 $ & HARPS \\
$ 7120.59836 $ & $  -341.80 $ & $    28.00 $ & $   -8.0 $ & $   37.0 $ & $   0.173 $ & HARPS \\
$ 7181.53193 $ & $   324.38 $ & $    24.00 $ & $ -136.0 $ & $   24.0 $ & $   0.759 $ & FEROS \\
$ 7185.51437 $ & $   228.38 $ & $    25.00 $ & $  -24.0 $ & $   24.0 $ & $   0.673 $ & FEROS \\
$ 7186.48111 $ & $  -235.62 $ & $    22.00 $ & $  125.0 $ & $   21.0 $ & $   0.380 $ & FEROS \\
$ 7187.48351 $ & $  -333.62 $ & $    25.00 $ & $  -36.0 $ & $   24.0 $ & $   0.114 $ & FEROS \\
$ 7190.47681 $ & $  -355.62 $ & $    24.00 $ & $   53.0 $ & $   24.0 $ & $   0.304 $ & FEROS \\
$ 7324.83438 $ & $   566.38 $ & $    19.00 $ & $  146.0 $ & $   18.0 $ & $   0.615 $ & FEROS \\
$ 7325.84444 $ & $  -219.62 $ & $    15.00 $ & $   86.0 $ & $   15.0 $ & $   0.354 $ & FEROS \\
$ 7327.85022 $ & $   386.38 $ & $    18.00 $ & $  137.0 $ & $   18.0 $ & $   0.822 $ & FEROS \\
$ 7403.83591 $ & $  -196.62 $ & $    15.00 $ & $   16.0 $ & $   15.0 $ & $   0.422 $ & FEROS \\
$ 7405.78818 $ & $   330.38 $ & $    17.00 $ & $   33.0 $ & $   17.0 $ & $   0.850 $ & FEROS \\
$ 7447.77082 $ & $   -15.62 $ & $    18.00 $ & $ -107.0 $ & $   18.0 $ & $   0.570 $ & FEROS \\


==> HATS655-001_rvtable.tex <==
$ 7119.69799 $ & $    57.38 $ & $    45.00 $ & $  -77.0 $ & $   53.0 $ & $   0.625 $ & HARPS \\
$ 7120.69688 $ & $    86.38 $ & $    19.00 $ & $  -83.0 $ & $   29.0 $ & $   0.884 $ & HARPS \\
$ 7181.59141 $ & $    72.23 $ & $    16.00 $ & $   54.0 $ & $   21.0 $ & $   0.686 $ & FEROS \\
$ 7182.52590 $ & $    28.23 $ & $    14.00 $ & $  -17.0 $ & $   18.0 $ & $   0.928 $ & FEROS \\
$ 7183.59764 $ & $   -86.77 $ & $    14.00 $ & $   13.0 $ & $   18.0 $ & $   0.206 $ & FEROS \\
$ 7184.48225 $ & $    -9.77 $ & $    15.00 $ & $   15.0 $ & $   19.0 $ & $   0.436 $ & FEROS \\
$ 7185.62553 $ & $   103.23 $ & $    21.00 $ & $  -43.0 $ & $   28.0 $ & $   0.732 $ & FEROS \\
$ 7186.57088 $ & $    62.23 $ & $    18.00 $ & $  -63.0 $ & $   24.0 $ & $   0.978 $ & FEROS \\
$ 7187.63960 $ & $   -48.77 $ & $    18.00 $ & $  -63.0 $ & $   24.0 $ & $   0.255 $ & FEROS \\
$ 7190.53242 $ & $   -32.77 $ & $    15.00 $ & $  -65.0 $ & $   19.0 $ & $   0.006 $ & FEROS \\
$ 7192.50171 $ & $   -36.77 $ & $    21.00 $ & $  -98.0 $ & $   28.0 $ & $   0.517 $ & FEROS \\
$ 7193.61040 $ & $    82.23 $ & $    15.00 $ & $    6.0 $ & $   19.0 $ & $   0.804 $ & FEROS \\
$ 7194.49223 $ & $   -27.77 $ & $    14.00 $ & $   16.0 $ & $   17.0 $ & $   0.033 $ & FEROS \\


==> newcommand_spec_multi_template.tex <==
%% GB's various newcommands for making editing easy for this specific paper

% This is the template version to be used for planets announced in a
% multi-planet paper. This file should be filled in separately for
% each planet in the paper. You should also find/replace the term
% xxxxB below with a unique identifier for each planet (e.g. xxxxB for
% the first one).  A version of this file should be saved with a
% unique name in the document directory for each planet, and all files
% should be processed into the newcommand_spec_multi.tex file using
% the scr/makenewcommand_spec_multi.sh script. This is done to allow
% you to reference planet information using commands like \hatcur{14}
% rather than \hatcurxxxxB. The newcommand_spec_multi.tex file so
% generated should not need to be edited or regenerated if changes are
% made to any of the planets parameters. Any changes should be made to
% the planet's own newcommand_spec.tex file.

% -------- Aliases specific to this paper/planet which should be edited -------

% The name of the host star and/or the planet:
\newcommand{\hatcurxxxxB}{HATS-40}
\newcommand{\hatcurbxxxxB}{HATS-40b}
\newcommand{\hatcurcxxxxB}{HATS-40c}

% The number used to index this system in the paper
\newcommand{\hatcurplanetnumxxxxB}{40}

\newcommand{\hatcurCCtwomassshortxxxxB}{06421710-2946365}

%\newcommand{\hatcurCCraxxxxB}{\ensuremath{08^{\mathrm h}39^{\mathrm m}31.82^{\mathrm s}}}  % right ascension
%\newcommand{\hatcurCCdecxxxxB}{\ensuremath{+47^{\mathrm d}21^{\mathrm m}07.4^{\mathrm s}}} % declination

\newcommand{\hatcurRVgammaabsxxxxB}{\hatcurRVgamma{\hatcurplanetnumxxxxB}}                           % Absolute Gamma velocity

\newcommand{\hatcurRVgammarelxxxxB}{\hatcurRVgamma{\hatcurplanetnumxxxxB}}                           % Relative Gamma velocity. Typically that of the Keck RVs.

\newcommand{\hatcurCCtassvixxxxB}{\ensuremath{NULL\pm NULL}}                  % TASS V-I

\newcommand{\hatcurSMEversionxxxxB}{i}                                       % Final SME version:i or ii?

% Isochrones used for this planet.
\newcommand{\hatcurisoshortxxxxB}{YY}
%\newcommand{\hatcurisoshortxxxxB}{Baraffe}
\newcommand{\hatcurisofullxxxxB}{Yonsei-Yale (YY)}
%\newcommand{\hatcurisofullxxxxB}{Baraffe}
\newcommand{\hatcurisocitexxxxB}{yi:2001}
%\newcommand{\hatcurisocitexxxxB}{baraffe:1998}

% Luminosity indicator used for this planet.
\newcommand{\hatcurlumindxxxxB}{\arstar}
%\newcommand{\hatcurlumindxxxxB}{Hip}s

% JHK filter type for the isochrone set used for this planet.
\newcommand{\hatcurjhkfilsetxxxxB}{ESO}
%\newcommand{\hatcurjhkfilsetxxxxB}{BB}
%\newcommand{\hatcurjhkfilsetxxxxB}{CIT}

% --------------------------------------------------------------------------
% The aliases below should not need editing, other than replaceing xxxxBx
% to whatever string.
% 
\newcommand{\hatcurSMEteffxxxxB}{\ifthenelse{\equal{\hatcurSMEversionxxxxB}{i}}{\hatcurSMEiteff{\hatcurplanetnumxxxxB}}{\hatcurSMEiiteff{\hatcurplanetnumxxxxB}}}
\newcommand{\hatcurSMEzfehxxxxB}{\ifthenelse{\equal{\hatcurSMEversionxxxxB}{i}}{\hatcurSMEizfeh{\hatcurplanetnumxxxxB}}{\hatcurSMEiizfeh{\hatcurplanetnumxxxxB}}}
\newcommand{\hatcurSMEzfehshortxxxxB}{\ifthenelse{\equal{\hatcurSMEversionxxxxB}{i}}{\hatcurSMEizfehshort{\hatcurplanetnumxxxxB}}{\hatcurSMEiizfehshort{\hatcurplanetnumxxxxB}}}
\newcommand{\hatcurSMEloggxxxxB}{\ifthenelse{\equal{\hatcurSMEversionxxxxB}{i}}{\hatcurSMEilogg{\hatcurplanetnumxxxxB}}{\hatcurSMEiilogg{\hatcurplanetnumxxxxB}}}
\newcommand{\hatcurSMEvsinxxxxB}{\ifthenelse{\equal{\hatcurSMEversionxxxxB}{i}}{\hatcurSMEivsin{\hatcurplanetnumxxxxB}}{\hatcurSMEiivsin{\hatcurplanetnumxxxxB}}}
\newcommand{\hatcurSMEvmacxxxxB}{\ifthenelse{\equal{\hatcurSMEversionxxxxB}{i}}{\hatcurSMEivmac{\hatcurplanetnumxxxxB}}{\hatcurSMEiivmac{\hatcurplanetnumxxxxB}}}
\newcommand{\hatcurSMEvmicxxxxB}{\ifthenelse{\equal{\hatcurSMEversionxxxxB}{i}}{\hatcurSMEivmic{\hatcurplanetnumxxxxB}}{\hatcurSMEiivmic{\hatcurplanetnumxxxxB}}}

